Who's Tracking Sensitive Domains?

We turn our attention to the elephant in the room of data protection, which is none other than the simple and obvious question: "Who's tracking sensitive domains?". Despite a fast-growing amount of work on more complex facets of the interplay between privacy and the business models of the Web, the obvious question of who collects data on domains where most people would prefer not be seen, has received rather limited attention. First, we develop a methodology for automatically annotating websites that belong to a sensitive category, e.g. as defined by the General Data Protection Regulation (GDPR). Then, we extract the third party tracking services included directly, or via recursive inclusions, by the above mentioned sites. Having analyzed around 30k sensitive domains, we show that such domains are tracked, albeit less intensely than the mainstream ones. Looking in detail at the tracking services operating on them, we find well known names, as well as some less known ones, including some specializing on specific sensitive categories.

==> sections/background.tex <==
\section{Background}\label{sec:background}


\subsection{Web Domain Classification}\label{sec:commercial-sys}

Definitions:

Web page classification is the process of assigning a web page to one or more predefined category
labels~\cite{Survey-Webpage-Classification}. In our case, the classification is a topical/subject classification, i.e.,
the five topics that are protected by GDPR. \gsnote{should we say here that other topics can be added for other
regulations, or if GDPR changes}

Many applications, e.g., searching, can be benefited by domain classification.
Mention the two main approaches: (1) supervised learning, (2) feature extraction. There is a huge literature here but we
are looking into how to use classification for particular, sensitive domains, appearing in data protection laws.


- Commercial tools, e.g., McAfee and Google Adwords are not transparent how they assign webpages to categories. Note
  that these tools were introduced to help advertisers select where their advertisements should be placed, and not to
identify sensitive domains.\gsnote{refer to the table 1 in intro}  

Our methodology can also be used to audit these categorization systems and our methodology is transparent instead of black
box (Datta paper~\cite{Datta-discrimination:2018})

It has been reported that classification based on generic categories, e.g., AdWords, McAfee etc. is not
accurate~\cite{Mobile-Apps-NDSS2018}.

\gsnote{the following can go to the intro}
- Discuss the story of insurance red lining~\cite{Wired-insurance-algos}. 

The algorithm can discriminate: Illegal to exclude audiences based on protected categories (eg Facebook anti-discrimination policy).




\subsection{Tracker Detection}\label{sec:academic-sys}

Academic literature and systems

-- General detection studies~\cite{openWPM-englehardt2016census,Mayer_2012,WebTracking-over-years}. open questions: do specialized trackers exist? is there a cross-tracking~\cite{DE-vs-Facebook}? 

-- Studies pertaining to tracking on sensitive domains. At most, the matter occupies a small section in more general measurement studies around tracking
such as~\cite{Mayer_2012,Mobile-Apps-NDSS2018,CoNEXT2015-Following,Iordanou:GDPR-IMC2018}.

-Domain specific studies (not as generic and practical as ours), e.g., Facebook \gsnote{should we cite
this:}\cite{Unveiling-Facebook-Exploitation}, Mobile~\cite{Mobile-Apps-NDSS2018,preinstalled-Android-sw,Narseo_2012} 
and PII information leakage in mobiles~\cite{Leung_2016,ReCon}


\nlnote{Cut this out (better) or move to background}
Discussion: incognito mode, i.e., a mode where the browser does not record the browsing activity of the user to mitigate
tracking, is not a good proxy to infer sensitive domains. A study in 2010 showed that incognito mode is used for regular
browsing, including shopping and news%~\cite{private-browsing-2010}. 
Survey studies show that, over time, more users are aware of
the incognito mode in browsers and increasingly use it as a popular browsing mode~\cite{Bursztein-survey,DuckDuckGo-survey}.  Moreover,
studies have shown that even in incognito mode the web browsing is not private and there is misconception about
this private browsing mode~\cite{incognito-problems,private-browsing-2010,Private-browsing-2014}.


Solution: We develop classifiers and we rely on crowdsourcing. As users are less willing to report information about the
content of the website, we rely on annotation of websites by the admins.

Caveat: Before we scale-up our analysis we select a set of manually selected seeds to avoid bias ans mis-classification.


==> sections/classification-old.tex <==
\section{Baseline Results}\label{sec:results}

\begin{table}[]
\caption{Main classifier dataset stats \cinote{Dataset stats for the main classifier using the DMOZ data}}
\label{tab:main_classifier_stats}
\begin{tabular}{|c|c|}
\hline
Category   & \# Labeled Samples \\ \hline
Health     & 1956               \\ \hline
Ethnicity  & 1956               \\ \hline
Religion   & 1956               \\ \hline
Sexual Or. & 1956               \\ \hline
Politics   & 1956               \\ \hline
Porn       & 781                \\ \hline
\end{tabular}
\end{table}

In this section we first demonstrate the accuracy of our classification of sensitive web sites and then perform a sensitivity analysis.

\subsection{Datasets}\label{sec:datasets}




Duration of the experiment:

{\bf Ethical considerations:} Add ethical consideration section.

For comparison with, typically non-sensitive, popular websites, we also crawl the top 2K? by Alexa. We decide to focus
only on the top 2K as the churn is small (10\%)~\cite{Alexa-stability:IMC2018} and we manually check that the variation
is even smaller (XX\%) during our crawling period, as some of the churn is due to websites that are owned by the same
organization, e.g., google.fr and google.ie.




\subsection{Classification Accuracy}

\nlnote{Some roadmap to be added here after the text is done}

\subsubsection{Text based classification}

Figure~\cite{} \cinote{Is better to refer to Table~\ref{table:overview-classifier-results}} depicts the accuracy of the classifier when operating on input provided by the text extracted from the landing page of a domain. The classifier of Sect.~\ref{} is configured to 
\nlnote{give the setup either here or on the legend of the corresponding figure. How many features are you using? 2K? lowercase=true, stop words=English, test-size= 30\%  
training-size=70\% (see also slide 31 and 51)}. 
\cinote{ Final Classifier Setup: \# of Features = 3k, lowercase = True, stop\_words = English, minimum\_word\_size\_in\_characters = 3, test\_size=3\%}
We see that under both Bag of Words \nlnote{Shouldn't we use an acronym for this} \cinote{Bag of Words (BoW)} and TF-IDF the accuracy of the classifier is pretty good. Bag of words accuracy: 82.6\%, TF-IDT accuracy: 84.24\%. Looking at the different sensitive categories we observe that XXX has the highest accuracy (YYY\%) whereas ZZZ is the most difficult one to classify (HHH\% accuracy). \cinote{We need to update the above numbers according to the final results.}

\nlnote{Can we provide some explanation about why some categories are easier to classify than others?} \cinote{Some examples: (1) Sexual orientation conflicts with Health (Sexually transmitted diseases such as HIV, etc.) (2) Ethnicity has a small correlation with religion. i.e. Arabs and people living in Middle-East are most probably Muslims, Similarly, Russian people are correlated with Christianity (Orthodox) and European with Christianity (Catholic). (3) Also Ethnicity is correlated with Politics due to the ISIS issues that we observe during the last few years.}

\cinote{Some comments on Figure~\ref{fig:effect-features-tf}: Sexual Orientation performance accuracy is the worst out of all 6 categories. The main reason is that we have multiple sub-categories of websites dedicated to a specific type of Sexuality, such as, websites dedicated to only gay men or lesbian women, etc. WRT Porn, we have the highest accuracy since almost all Porn websites follow the same theme, i.e. a list of video thumbnails and a short description using a specific "catchy" descriptions.}

\gsnote{Explain what a confusion matrix is. Explain that the darker the color the better. Refer to Figure~\ref{fig:confusion-matrix-content}(a).}

Table~\ref{table:top10-features} depicts the top 10 features used by the classifier under bag of word and TF-IDF \cinote{I only report the features using the TF-IDF in Table~\ref{table:top10-features}} in order to achieve the aforementioned accuracy. We observe that \nlnote{what can we say that is interesting here?} \cinote{We observe that in all categories we have only relevant keywords as the most predictive features.}

\begin{figure}[t]
	\centering

	
  	\subfloat[Bag of Words - Meta ] {{\includegraphics[width=.31\columnwidth]{figures/cm_bow_meta.pdf} }} \hspace{0.5mm} \hfill
  	%\qquad
	\subfloat[Bag of Words - Content ] {{\includegraphics[width=.31\columnwidth]{figures/cm_bow_content.pdf} }} \hspace{0.5mm} \hfill
  	%\qquad
	\subfloat[Bag of words - Meta + Content ]{{\includegraphics[width=0.31\columnwidth]{figures/cm_bow_meta_content.pdf} }}	\hfill
	\qquad
	\subfloat[TF-IDF - Meta ]{{\includegraphics[width=0.31\columnwidth]{figures/cm_tf_idf_meta.pdf} }} \hspace{0.5mm} \hfill
	%\qquad
	\subfloat[TF-IDF - Content ]{{\includegraphics[width=0.31\columnwidth]{figures/cm_tf_idf_content.pdf} }} \hspace{0.5mm} \hfill
	%\qquad
	\subfloat[TF-IDF - Meta + Content ]{{\includegraphics[width=0.31\columnwidth]{figures/cm_tf_idf_meta.pdf} }} \hfill
    \caption{ place the confusion matrices and the accuracies: (a) only content:
top-left: slide 18: Bag of words-content, 82.64\%, 
bottom-left: slide 19: TF-IDF model - Only Content, 84.24\%  
(b) all:
top-right: slide 16: Bag of words model - ALL, 83.8\%,
bottom-right: slide 17: TF-IDF model - ALL, 85.6\%,
\gsnote{we may want to add the porn and coppa here}
\cinote{I include overall 6 CMs. WRT feature engineering algorithm, we have Bag of Words and TF-IDF. For each feature engineering algorithm I report the CM using 3 different inputs. Only Meta, only Content, and Meta + Content}
}
\label{fig:confusion-matrix-content}
\end{figure}


%\begin{figure}[t]
%    \centering
%\includegraphics[width=.3\columnwidth]{test-figures/t.pdf}
%\caption{ place the confusion matrices and the accuracies: (a) only content:
%top-left: slide 18: Bag of words-content, 82.64\%, 
%bottom-left: slide 19: TF-IDF model - Only Content, 84.24\%  
%(b) all:
%top-right: slide 16: Bag of words model - ALL, 83.8\%,
%bottom-right: slide 17: TF-IDF model - ALL, 85.6\%,
%\gsnote{we may want to add the porn and coppa here}}
%\label{fig:confusion-matrix-content}
%\end{figure}


\subsubsection{Meta-information based classification}

Having seen that classification based on the textual content of the landing page of a domain can tell with high accuracy whether it belongs to a certain sensitive category, we turn to ask whether the same can be done more efficiently. Specifically, we would like to asses whether such classification can be achieved using only the meta information of domains, including fields such as \nlnote{add} \cinote{the website title, description, keywords, etc. found under the HTML \textsl{<meta>} tag}. If this were the case, then there would be a big advantage in terms of efficiency/scalability of training and applying the classifier since the meta-information has orders of magnitude smaller volume than the actual content of a page, even if only its tectual part. \nlnote{Can we put some numbers here about the volume of text vs. meta-information?} \cinote{ TODO: Count the string length for META Vs Content. }

Table~\ref{table:overview-classifier-results} shows that using only meta-information the classification drops in efficiency for all sensitive categories under both BoW and TF-IDF compared to using the full text of a page. At best it is as high as XXX for \nlnote{name the sensitive category}, but it can be as low as YYY for \nlnote{name the sensitive category} \cinote{In case we need to report numbers per sensitive category, we have the results in Google Drive presentation - Slides 93 - 94 (see F1 Scores)}.

\nlnote{Should we say something about which is the most useful feaure in this case. If yes, just in text, no table.}

\subsubsection{Combining text and meta-information}

Next we attempt to see if training using both meta-information and text can improve the classification accuracy compared to using text only. Figure~\ref{} shows that his is indeed the case, but the gains are rather marginal -- typically less than XXX\% improvement. 
\cinote{And again... In case we need to report numbers per sensitive category, we have the results in Google Drive presentation - Slides 93 - 94 (see F1 Scores)}.

\begin{table}[t]
\caption{Top 10 features (out of the 3K) in the sensitive categories. The classifier is  using as an input the websites meta-data and content, and the TF-IDF algorithm for feature engineering.\gsnote{keep it if there is space, o.w. in the text}}
\label{table:top10-features}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
A/A & Health    & Ethnicity  & Religion  & Sexual Or. & Politics   & Porn  \\ \hline
1   & Cancer    & Native     & Church    & Gay        & Party      & Porn  \\ \hline
2   & Disease   & Indian     & God       & Lesbian    & Democrats  & Sex   \\ \hline
3   & Health    & American   & Bible     & Sex        & News       & Video \\ \hline
4   & Treatment & Language   & Christian & LGBT       & Government & Teen  \\ \hline
5   & Syndrome  & Tribe      & Faith     & Queer      & State      & Free  \\ \hline
6   & Symptoms  & History    & Prayer    & Bisexual   & Political  & Girls \\ \hline
7   & Patients  & People     & Holy      & Community  & Liberal    & Anal  \\ \hline
8   & Research  & Culture    & Catholic  & HIV        & Election   & Pussy \\ \hline
9   & Clinical  & Tribal     & Religious & Pride      & Parliament & Hot   \\ \hline
10  & Care      & Indigenous & Love      & Events     & Labour     & Big   \\ \hline
\end{tabular}
}
\end{table}


\subsubsection{Classification based on third party domain presence}

Last, we attempt to see if classification is possible based on the presence of certain trackers. Basically, we would like to see if the presence of trackers can be used as a finger print for classifying domains into categories. 

This does not seem to be the case. \nlnote{Can we do this?: Despite the fact that the presence of trackers can be used to uniquely identify a website with high accuracy (XXX\%), it is not sufficient for classifying whether it belongs to a certain category among the sensitive ones we consider}.  

\gsnote{
Third parties/trackers all, (slides 32+33), or annotated with the
level, (slides 34+45), are not good
features for this classification.}
\cinote{My guess here is that even if we have a specialized tracker that operates exclusively on a specific sensitive category due to low (domains) coverage the classifier is not performing well. At the end the classifier is trying to identify a feature (or combination of features) that is almost always present in a specific classification class (our case, website).}

\subsubsection{Summary}

Table~\ref{table:overview-classifier-results} summarizes our results on classification accuracy. We conclude that \emph{to classify accurately sensitive domains one needs to use at least their textual content. Using meta-information alone is not enough, whereas combining meta-information with textual content yields a small improvement over content alone. Fingerprint based on based on the presence of tracking domains does not work.} \cinote{We can claim the following. Based on our final results we observe that the combination of Meta + Content provide the highest accuracy (85.66\%). We opt to these combination since the size of the meta data is relatively small compare to the size of the actual content imposing minimal overheat to our training phase and gaining an additional 1.36\% accuracy improvement.}


\begin{table}[t]
\caption{Overview of the accuracy for different feature sources and feature types (Bag of Words and TF-IDF)
\cinote{Fix the accuracy based on the confusion matrix figure, we have some inconsistency due to decimal round ups.}
}
\label{table:overview-classifier-results}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
Feature Source & Bag of Words & TF-IDF\\ \hline
Third-party domains (TPD) & 43.28 & 44.26\\ \hline
 TPD with Levels (TPD\_LVL) & {\color{red} 42.27} & 43.19 \\ \hline
 Meta (M) & 77.92 & 77.10 \\ \hline
 Content (C) & 79.92 & 84.29\\ \hline
 M + C & 81.50 & {\color{blue} \textbf{85.65}}\\ \hline
 M + C + TPD & 81.44 & 85.59\\ \hline
 M + C + TPD\_LVL & 81.47 & 85.62 \\ \hline
\end{tabular}
}
\end{table}


\subsection{Sensitivity Analysis}

Next we examine the sensitivity of accuracy on the number of features used and on the quality of the initial training seed. We report only for combined meta-information and textual content classification \nlnote{verify} that achieves the highest accuracy.

\subsubsection{Number of features}


\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/Features_num.pdf}
\caption{\cinote{Bag of Words - Remove this one and use the TF-IDF one} Figure for results in slides 48, 49, 50 -- results for the best feature source and feature type. x-axis: \# of
features, y-axis: accuracy. 5 lines, one for H, E, R, S, P (we can add porn and COPPA).}
\label{fig:effect-features}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/Features_num_tf.pdf}
\caption{\cinote{TF-IDF dataset}Figure for results in slides 48, 49, 50 -- results for the best feature source and feature type. x-axis: \# of
features, y-axis: accuracy. 5 lines, one for H, E, R, S, P (we can add porn and COPPA).}
\label{fig:effect-features-tf}
\end{figure}

We vary the number of features used in training the classifier. Figure~\ref{fig:effect-features} shows that from XXX-YYY features and on wards the classification improvement is marginal. At the same time using more features has an impact on training time \nlnote{Can we give some numbers here.} therefore from now on we will be using classification with XXX features. \cinote{See Table~\ref{table:execution_times}}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Execution time for feature engineering and training time using different combination of inputs and number of features}
\label{table:execution_times}
\begin{tabular}{|c|r|c|c|c|c|}
\hline
\multirow{2}{*}{Input}       & \multicolumn{1}{c|}{\multirow{2}{*}{\# Features}} & \multicolumn{2}{c|}{Feature Eng. Time} & \multicolumn{2}{c|}{Training Time} \\ \cline{3-6} 
                             & \multicolumn{1}{c|}{}                             & BoW               & TF-IDF             & BoW              & TF-IDF          \\ \hline
\multirow{3}{*}{Meta (M)}    & 1 000                                             & 920ms             & 359ms              & 18.6ms           & 16.5ms          \\ \cline{2-6} 
                             & 10 000                                            & 893ms             & 367ms              & 19.2ms           & 17.9ms          \\ \cline{2-6} 
                             & 100 000                                           & 878ms             & 368ms              & 26.4ms           & 23.8ms          \\ \hline
\multirow{3}{*}{Content (C)} & 1 000                                             & 13.4s             & 12.9s              & 28.1ms           & 21.7ms          \\ \cline{2-6} 
                             & 10 000                                            & 13.1s             & 12.9s              & 48.3ms           & 39.4ms          \\ \cline{2-6} 
                             & 100 000                                           & 13.2s             & 13.1s              & 91.3ms           & 79.4ms          \\ \hline
\multirow{3}{*}{M + C}       & 1 000                                             & 13.2s             & 13.0s              & 26.7ms           & 22.8ms          \\ \cline{2-6} 
                             & 10 000                                            & 13.2s             & 13.1s              & 44.4ms           & 32.8ms          \\ \cline{2-6} 
                             & 100 000                                           & 13.4s             & 13.4s              & 86.2ms           & 67.6ms          \\ \hline
\end{tabular}
\end{table}

%Can a small but very robust see make a difference, see applications to other domains:~\cite{The-Wisdom-of-the-Few}; it is
%important to select well the seeds.

\begin{figure}[t]
\centering
\includegraphics[width=.3\columnwidth]{test-figures/t.pdf}
\caption{Accuracy of the classifier in the presence of noise. x-axis:
percentage of noise (not related websites), y-axis: accuracy. 5 lines, one for H, E, R, S, P (we can add port and COPPA).
\cinote{TODO: Create this figure after section 5 results (Trackers) since it will take some time to create it.}}
\label{fig:robustness}
\end{figure}


\subsubsection{Noise on the seeding set} 

A fundamental characteristic of our classification approach is the combination of crowdsourcing with so call ``wisdom of the few''~\cite{The-Wisdom-of-the-Few}: we rely on a crowdourced index of terms for websites provided by DMOZ \cinote{Instead of DMOZ use Curlie (http://curlie.org/). DMOZ is not active anymore.} but rely on expert's opinion to select among them a small seed set of domains that truly exemplify a sensitive category. We have shown so far that even a very limited seed set suffices to drive the rest of our methodology, in the end, achieved a high classification accuracy. In this section we look at the effect of ``noise'' on the seed test, \ie, we look at the impact on classification accuracy on mistakes on the part of the expert in selecting domains as seed. To do that, we start from the carefully selected seed sets used in the previous examples and add noise progressively by substituting a percentage of the original domains with randomly selected ones from XXX. Figure~\ref{} shows that \nlnote{To be done} \cinote{TODO: First graph to create after finishing Trackers results (Next Section).}  

%\begin{figure}[t]
%\centering
%\includegraphics[width=.2\columnwidth]{test-figures/t.pdf}
%\caption{Accuracy \todo{one Alexa category (top 2K websites in the category) -- Health}; later we can add the confusion
%matrix for all categories}
%\label{fig:off-the-shelf-tools}
%\end{figure}



\nlnote{This should go to methodology if you have lots to say or drop being separate subsection}
\subsection{Limitations}

mention any limitation or other advanced features that we do not consider, e.g., rendering of ads etc.


\nlnote{This needs to go elsewhere or removed}
\subsubsection{The failure of off-the-shelf tools:}  Show that with top 2k Alexa (per
category) you get crap (same with McAfee and GoogleAds?). \cinote{ TODO: Include this after noise inclusion and classification stability results graph. }

%LATER: show confusion matrix for all categories (needs to run again for all the sensitive categories)
%For this we show the confusion matrix
%(that we used for our classifier) with using the top XX websites based on McAfee, Google Adwords, alexa per category,
%see Figure~\ref{fig:off-the-shelf-tools} -- add confusion matrix.





%Since it is binary classifier this does not make sense:
%\subsection{Performance vs complexity of different classifiers}\label{sec:performance-complexity}
%
%\begin{figure}[t]
%\centering
%\includegraphics[width=.3\columnwidth]{test-figures/t.pdf}
%\caption{ROC diagrams TPD, TPD\_LVL, Meta, Content, Meta + Cont., Meta + Cont. + TPD, Meta + Cont. +
%TPD\_LVL;  one for: H, E, R, S, P (we can add port and COPPA).\gsnote{let's discuss the details of this figure}}
%\label{fig:performance-vs-complexity}
%\end{figure}
%
%Precision and Recall; Figure~\ref{fig:performance-vs-complexity} (slides 66, 67)




==> sections/implications.tex <==
\section{Implications}


- investigation: addressing complaints by regulators

- audit/inform advertisers

- inform users, visit of sensitive webpages, existence of specialized trackers, existence of csync

- adding features for users, e.g., avoid indexing for search engines



==> sections/manual.tex <==
\subsection{Manual Seeding}\label{sec:manual}

We rely on classification annotated by the owners of the webpage. For our study we rely in DMOZ~\cite{DMOZ-dataset}: 3.6M web-pages
annotated with short description. 

DMOZ has XX categories. We manually identify the categories that are closely related
to the sensitive category labels. 

In this study we focus on the 5 GDPR categories, namely: Health, Religion, Sexual, Ethnicity
Politics. A sixth category is biometric data that we do not investigate in this study. Note, that can re-use the same
methodology if the list of categories is extended or change, e.g., Porn, COPPA~\todo{add citation}, a law created to protect the privacy of
children under 13 (see Section~\ref{sec:results}).

We focus on the top subcategories that are generally accepted as sensitive, i.e., AIDS in health, left and right in
politics, etc. We manually confirm that this is a sensitive topic, \todo{give an example, e.g., health - cancer -
specific cancer}. \todo{should we also cite this one:}\cite{Automated-Classification-DMOZ}.

example: FILTER = (Health and Conditions-and-Diseases) NOT (Animal, Allergies, Wounds-and-Injuries)

We provide XX websites for each category (maybe we can present the subcategories and the websites in the Appendix).

%Steps:
%
%\begin{enumerate}
%
%\item Identify the first x for each sensitive category (table to be approved) [check complaints related to GDPR/court
%cases/Google GDPR] - Check EU stats related to GDPR; how the ``traditional'' categorization tools classify them?
%
%\item Check if we can get the seeds from the GDPR complains lists and use those for classification
%
%\item Otherwise do it manually
%
%\item Which websites appear mostly in the incognito mode/block lists? Check overlaps 1-4
%
%\end{enumerate}




==> sections/table-with-examples.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{Top 10 websites per sensitive categories and how relevant they are.\gsnote{we may remove this table or discuss
it later, when we discuss the need for our classifier, and compare the performance of our classifier and simple
approaches like this}}
\label{table:misleading-websites-tools}
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{|l|lp{4cm}|lp{4cm}|lp{4cm}|lp{4cm}|lp{4cm}|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{A/A}} & \multicolumn{2}{c|}{Health - /Top/Health/Conditions\_and\_Diseases}                                                                                                                                                                                                   & \multicolumn{2}{c|}{Religion - /Top/Society/Religion\_and\_Spirituality}                                                                                                                                                                                                                     & \multicolumn{2}{c|}{Sexual Orientation - /Top/Society/Gay,\_Lesbian,\_and\_Bisexual}                                                                                                                                                                                   & \multicolumn{2}{c|}{Ethnicity - /Top/Society/Ethnicity}                                                                                                                                                                                                                                                                     & \multicolumn{2}{c|}{Politics - /Top/Society/Politics}                                                                                                                                                   \\
\multicolumn{1}{|c|}{}                     & \multicolumn{1}{c}{Domain} & \multicolumn{1}{c|}{Description}                                                                                                                                                                                                         & \multicolumn{1}{c}{Domain} & \multicolumn{1}{c|}{Description}                                                                                                                                                                                                                                & \multicolumn{1}{c}{Domain} & \multicolumn{1}{c|}{Description}                                                                                                                                                                                                          & \multicolumn{1}{c}{Domain} & \multicolumn{1}{c|}{Description}                                                                                                                                                                                                                                                               & \multicolumn{1}{c}{Domain} & \multicolumn{1}{c|}{Description}                                                                                                                                           \\ \hline
1                                          & nih.gov                    & US Government department in charge of medical research.                                                                                                                                                                                  & jw.org                     & Jehovah's Witnesses. Profile, beliefs, activities, publications, contact information.                                                                                                                                                                           & queerty.com                & Coverage of media, politics, and celebrities.                                                                                                                                                                                             & soompi.com                 & Soompi is the largest community site for English speaking fans of Asian pop culture and entertainment such as Korean dramas and music. It has also grown into the largest Asian American site on the web.                                                                                      & slate.com                  & Online magazine of news and commentary on culture and politics                                                                                                             \\ \cline{2-11} 
2                                          & webmd.com                  & Resource for consumers, physicians, nurses, and educators. Includes news, chat forums, health quizzes and consumer product updates                                                                                                       & biblegateway.com           & Search the Bible in English, German, Swedish, Latin, French, Spanish, Portuguese, Italian, Tagalog, and Norwegian.                                                                                                                                              & out.com                    & A gay and lesbian perspective on style, entertainment, fashion, the arts, politics, culture, and the world at large.                                                                                                                      & bet.com                    & Network programming schedule for the BET network.                                                                                                                                                                                                                                              & infowars.com               & The web page of syndicated radio host Alex Jones. Conspiracy-tinted site containing strong opposition to socialism, communism, and the New World Order.                    \\ \cline{2-11} 
3                                          & mayoclinic.org             & Clinical experts provide current medical information and news on health topics.                                                                                                                                                          & lds.org                    & Official site of the church headquartered in Salt Lake City since 1847. Scriptural and genealogical resources, news and announcements.                                                                                                                          & autostraddle.com           & News, entertainment and culture for lesbian, bisexual and otherwise-inclined ladies on the edge.                                                                                                                                          & thesource.com              & For 20 years, The Source has been the leading international voice for the ever-evolving world of Hip-Hop music, culture and politics.                                                                                                                                                          & salon.com                  & The Web s best source and online magazine for smart, timely, lively original reporting and commentary on news and politics, business and entertainment, culture, and life. \\
4                                          & cdc.gov                    & Mission is to promote health and quality of life by preventing and controlling disease, injury, and disability.                                                                                                                          & biblehub.com               & Each verse is listed on one page in several English translations.                                                                                                                                                                                               & advocate.com               & The U.S. based national gay and lesbian news magazine. Includes the GSK pride guide, forums, and links related to articles.                                                                                                               & basnews.com                & Current news in Iraq Kurdistan                                                                                                                                                                                                                                                                 & weforum.org                & The Foundation organizes the Davos meeting of political and business leaders.                                                                                              \\
5                                          & psychologytoday.com        & Featured columns on relationships, mental health education, and work related issues. Recent mental health news and archives.                                                                                                             & familysearch.org           & The Church of Jesus Christ of Latter-day Saints provides an online search of the millions of names in its International Genealogical Index, and of genealogical Web sites.                                                                                      & datalounge.com             & Forum in existence for more than a decade to discuss any topic. Required paid subscription to access at peak times.                                                                                                                       & essence.com                & Issued monthly, focusing on women's issues.                                                                                                                                                                                                                                                    & dailykos.com               & Daily weblog with political analysis on US current events from a liberal perspective.                                                                                      \\
6                                          & *myfitnesspal.com          & Free online food diary, calorie counter with large food database.                                                                                                                                                                        & biblestudytools.com        & Resources for conducting word, verse, and topic searches in many Bible versions, Greek and Hebrew lexicons, commentaries, concordances, and biblical dictionaries. Includes church history and sermon helps.                                                    & towleroad.com              & "influential...must read" Washington Post. Winner, Best LGBT -- Weblog Awards. Weblog of Year, Gay Bloggies. General Interest. Different Insights. Hot guys in the news.                                                                  & soas.ac.uk                 & University of London is the world's leading centre for the study of a highly diverse range of subjects concerned with Asia, Africa and the Middle East.                                                                                                                                        & nationalreview.com         & Up-to-the-minute conservative commentary on politics, news, and culture. I                                                                                                 \\
7                                          & who.int                    & World Health Organization                                                                                                                                                                                                                & gotquestions.org           & Got Questions? The Bible has answers! We'll find them for you! Bible Questions Answered by GotQuestions.org                                                                                                                                                     & lgbtqnation.com            & U.S. news, opinions, art and culture articles.                                                                                                                                                                                            & jewishvirtuallibrary.org   & Encyclopedia of Jewish history and culture covering everything from anti-Semitism to Zionism.                                                                                                                                                                                                  & townhall.com               & Conservative political news and opinion, editorial cartoons, political analysis and commentary.                                                                            \\
8                                          & medlineplus.gov            & Health information from the National Library of Medicine. Easy access to Medline and Health topics, medical dictionaries, directories and publications.                                                                                  & jpost.com                  & Daily news and events from Israel's leading English national broadsheet.                                                                                                                                                                                        & hrc.org                    & Works for lesbian, gay, bisexual and transgender equal rights by lobbying the federal government, educating the public, participating in election campaigns, organizing volunteers, and providing training at the state and local levels. & okayplayer.com             & An online community featuring recording artists whose official Internet sites reside there.                                                                                                                                                                                                    & newsmax.com                & News, investigations and commentaries.                                                                                                                                     \\
9                                          & medscape.com               & Features medical journal articles, images, case reports, medical news, free Medline, CME, and drug searching.                                                                                                                            & *astro.com                 & Offers a large selection of charts, horoscopes and information. A database of over 200,000 cities with complete timezone and daylight savings time information.                                                                                                 & gaystarnews.com            & Rolling 24/7 global gay news website for the lesbian, gay, bisexual and transgender community.                                                                                                                                            & vibe.com                   & Covers hip hop/urban culture with a focus on music. Articles, interviews, and subscription information.                                                                                                                                                                                        & gallup.com                 & Gallup.com provides data-driven news to leaders, business executives, and decision makers worldwide.                                                                       \\
10                                         & kaiserpermanente.org       & USA  A not-for-profit organization serving members in several states and Washington, DC. It operates as a working partnership of two organizations: Kaiser Foundation Health Plan and Hospitals, and the Permanente Medical Groups. & islamicfinder.org          & Given a location, the site provides local prayer times and a list of masjids, Islamic centers and organizations, and Islamic-owned businesses nearby.                                                                                                           & newnownext.com             & Pop culture daily news, celebrity gossip, and photos.                                                                                                                                                                                     & tki.org.nz                 & A bilingual portal-plus web community which provides quality assured educational material for New Zealand teachers, school managers, and the wider education community.                                                                                                                        & wnd.com                    & Independent news source with emphasis on aggressive investigative reporting.                                                                                               \\
11                                         & nhs.uk                     & Your complete guide to conditions, symptoms and treatments, including what to do and when to get help.                                                                                                                                   & *horoscope.com             & Free daily horoscopes, free daily Chinese astrological forecast, unique daily celebrity astro gossip section, natal charts, astro-match.                                                                                                                        & outsports.com              & Gay sports news, commentary, photos and videos.                                                                                                                                                                                           & irishcentral.com           & Whether you are looking for Irish news, Irish entertainment, Irish sport, or Irish stars- IrishCentral.com is the best source for everything Irish.                                                                                                                                            & reason.com                 & A libertarian magazine covering politics, culture, and ideas through a mix of news, analysis, commentary, and reviews.                                                     \\ \hline
12                                         & bmj.com                    & Electronic version of the BMJ. Publish accessible information that will help doctors improve their practice and will influence the international debate on health. Access is free to all.                                                & desiringgod.org            & God-centered resources from the ministry of John Piper — sermons, books, articles, audio and video, free of charge.                                                                                                                                             & glaad.org                  & Promotes fair and accurate representation of gay people in                                                                                                                                                                                & tamilcube.com              & Your one-stop portal for Tamil, Hindi and Malay language online resources! Offers Tamil translation service, online and mobile dictionaries, Tamil test papers, Tamil eBooks, tutor matching and many more.                                                                                    & commondreams.org           & Breaking news \& views for the Progressive Community                                                                                                                       \\ \hline
13                                         & medicinenet.com            & Describes conditions, diseases, tests, and procedures, with a medical dictionary.                                                                                                                                                        & blueletterbible.org        & Searchable King James Version, with Greek text for each New Testament verse in graphics form (no font software needed, but no breathings or accents).                                                                                                           & instinctmagazine.com       & An LGBTQ site dedicated to bringing you the latest and greatest news and entertainment.                                                                                                                                                   & yellowbridge.com           & Includes news, literature, language, and humor from a Chinese-American perspective.                                                                                                                                                                                                            & marxists.org               & The most complete database of Marxism hitherto made.                                                                                                                       \\ \hline
14                                         & *menshealth.com            & Site contains daily tips and articles on fitness, nutrition, relationships, sex, career and lifestyle.                                                                                                                                   & *alrajhibank.com.sa        & The largest Islamic Bank in the world. Al Rajhi Bank offers number of retail banking solutions such as Personal, Auto and Home finance, in addition to corporate financial solutions.                                                                           & afterellen.com             & Reviews and commentary on the representation of lesbians and bisexual women in entertainment and the media, including television, movies, books, and celebrity news.                                                                      & blackenterprise.com        & Information regarding entrepreneurship, technology, personal finance and other minority business issues.                                                                                                                                                                                       & thenation.com              & News and analysis on politics and culture from the left.                                                                                                                   \\ \hline
15                                         & verywellhealth.com         & Verywell Health is an award-winning resource for reliable, understandable, and up-to-date information on the medical topics that matter most to you.                                                                                     & chabad.org                 & The movement's flagship site. Provides thousands of articles, audio and video clips, daily Torah classes, Shabbat candle-lighting times, Ask-the-Rabbi, magazine, Parshah, primary Jewish texts including the Bible, global Jewish calendar, searchable library & gaycities.com              & The comprehensive gay travel guide built by and for the gay                                                                                                                                                                               & Ebony.com                  & Largest Black owned publishing company. Produces a variety of publications, magazines and television production, such as EBONY and JET magazines, along with Fashion Fair cosmetics and hair care products Ebony magazine is one of the oldest African American magazines and most successful. & newrepublic.com            & Razor-sharp analysis on the world of politics and culture.                                                                                                                 \\ \hline
\end{tabular}
}
\end{table*}



